AttenGluco: Multimodal Transformer-Based Blood Glucose Forecasting on AI-READI Dataset

Diabetes is a chronic metabolic disorder characterized by persistently high blood glucose levels (BGLs), leading to severe complications such as cardiovascular disease, neuropathy, and retinopathy. Predicting BGLs enables patients to maintain glucose levels within a safe range and allows caregivers to take proactive measures through lifestyle modifications. Continuous Glucose Monitoring (CGM) systems provide real-time tracking, offering a valuable tool for monitoring BGLs. However, accurately forecasting BGLs remains challenging due to fluctuations due to physical activity, diet, and other factors. Recent deep learning models show promise in improving BGL prediction. Nonetheless, forecasting BGLs accurately from multimodal, irregularly sampled data over long prediction horizons remains a challenging research problem. In this paper, we propose AttenGluco, a multimodal Transformer-based framework for long-term blood glucose prediction. AttenGluco employs cross-attention to effectively integrate CGM and activity data, addressing challenges in fusing data with different sampling rates. Moreover, it employs multi-scale attention to capture long-term dependencies in temporal data, enhancing forecasting accuracy. To evaluate the performance of AttenGluco, we conduct forecasting experiments on the recently released AIREADI dataset, analyzing its predictive accuracy across different subject cohorts including healthy individuals, people with prediabetes, and those with type 2 diabetes. Furthermore, we investigate its performance improvements and forgetting behavior as new cohorts are introduced. Our evaluations show that AttenGluco improves all error metrics, such as root mean square error (RMSE), mean absolute error (MAE), and correlation, compared to the multimodal LSTM model. AttenGluco outperforms this baseline model by about 10% and 15% in terms of RMSE and MAE, respectively.

==> Sections/xx_lit_rev_tbl.tex <==
% \begin{table*}[ht]
% \centering
% \caption{Summary of Methods, Limitations, and Data Constraints}
% \label{tab:summary}
% \begin{tabular}{p{2.2cm} p{2.2cm} p{2.8cm} p{3.0cm} p{3.0cm} p{2.5cm}}
% \hline
% Method & Examples & Key Features & Limitations & Dataset Used & Public Avail. \\
% \hline
% ARIMA & \cite{xie2020benchmarking} & Straightforward time-series & 5--15\% higher RMSE vs. ML; struggles with nonlinearities \cite{xie2020benchmarking, mujahid2021machine} & Mixed or partial data, not fully specified & Generally N/A \\
% ML (SVM, RF, ANN) & \cite{xie2020benchmarking, mujahid2021machine} & Adaptable to moderate complexities & Still limited in long-term temporal modeling & Often partial or specialized sets \cite{xie2020benchmarking} & Typically not public \\
% LSTM (RNN) & \cite{chung2014empirical, shuvo2023deep} & Gating to mitigate gradient issues & High computational overhead; sensor drift and user non-adherence hamper real-world use \cite{kong2024unlocking} & OhioT1DM (Type 1) \cite{shuvo2023deep} & OhioT1DM is public \\
% GRU (RNN) & \cite{chung2014empirical, Elsayed_2019} & Faster convergence than LSTM & Incomplete logs, inconsistent data sampling remain problematic \cite{kong2024unlocking} & General time-series in \cite{Elsayed_2019} & N/A \\
% TFT & \cite{zhu2023edge, acuna2023analyzing, zhang2024multi} & Multi-head attention, gating & No cross-attention, large-data requirement \cite{acuna2023analyzing} & Custom/varied sets (type unspecified) & Partial \\
% Gluformer & \cite{sergazinov2023gluformer} & Uncertainty quantification & 1--2 mg/dL improvement, lacks multi-head/cross-attention for multimodal integration \cite{sergazinov2023gluformer} & Custom/partial data & Unknown \\
% \hline
% \end{tabular}
% \end{table*}
